Introducing SESHAT: A Tool for Object Classification from JWST Catalogs

JWST's exquisite data have opened the doors to new possibilities in detecting broad classes of astronomical objects, but also to new challenges in classifying those objects. In this work, we introduce SESHAT, the Stellar Evolutionary Stage Heuristic Assessment Tool for the identification of Young Stellar Objects, field stars (main sequence through asymptotic giant branch), brown dwarfs, white dwarfs, and galaxies, from any JWST photometry. This identification is done using the machine learning method XGBoost to analyze thousands of rows of synthetic photometry, modified at run-time to match the filters available in the data to be classified. We validate this tool on real data of both star-forming regions and cosmological fields, and find we are able to reproduce the observed classes of objects to a minimum of 85\% recall across every class, with all available data, without additional information on the ellipticity or spatial distribution of the objects. Furthermore, this tool can be used to test the filter choices for JWST proposals by verifying whether the chosen filters are sufficient to identify the desired class of objects. SESHAT is released as a Python package to the community for general use.

==> old_sesna_app.tex <==

\begin{figure*}[h]
    \centering
    \includegraphics[width=0.75\linewidth]{AFGL_490_cm.pdf}
    \includegraphics[width=0.75\linewidth]{AFGL_490_hersch_col.pdf}
    \caption{
    \textit{Top}: Confusion matrix for AFGL 490 (part of test set). \textit{Bottom}: The grayscale image is extinction from \citet{Chiang2023} with the YSOs identified in this work and SESNA labeled with gold stars, the YSOs only identified by SESHAT labeled with red circles, and the YSOs only identified in SESNA labeled with red squares.
    %Contours from the extinction maps of \citet{Dobashi2005}: $A_V=1$ mag in white, $A_V=2$ mag in light gray, $A_V = 5$ mag in dark gray, and $A_V=10$ mag in black.
    \label{fig:afgl490}}
\end{figure*}


\begin{figure*}[h]
    \centering
    \includegraphics[width=0.75\linewidth]{Aquila_cm.pdf}
    \includegraphics[width=0.75\linewidth]{Aquila_hersch_col.pdf}
    \caption{The same as Figure~\ref{fig:afgl490}, but now for the Aquila star-forming region, which is part of the test set. 
    }
    \label{fig:aquila}
\end{figure*}


\begin{figure*}[h]
    \centering
    \includegraphics[width=0.75\linewidth]{Auriga-California_cm.pdf}
    \includegraphics[width=0.75\linewidth]{Auriga-California_hersch_col.pdf}
    \caption{The same as Figure~\ref{fig:afgl490}, but now for the Auriga-California star-forming region, which is part of the test set. }
    \label{fig:aur-cal}
\end{figure*}


\begin{figure*}[h]
    \centering
    \includegraphics[width=0.75\linewidth]{Cepheus_Flare_cm.pdf}
    \includegraphics[width=\linewidth]{Cepheus_Flare_hersch_col.pdf}
    \caption{The same as Figure~\ref{fig:afgl490}, but now for the Cepheus Flare region, which is part of the test set. The observations were taken with significant separation to require separate cutouts.}
    \label{fig:ceph-flare}
\end{figure*}


\begin{figure*}[h]
    \centering
    \includegraphics[width=0.75\linewidth]{Cepheus_OB3_cm.pdf}
    \includegraphics[width=0.75\linewidth]{Cepheus_OB3_hersch_col.pdf}
    \caption{The same as Figure~\ref{fig:afgl490}, but now for the Cepheus OB3 region, which is part of the test set. }
    \label{fig:ceph-ob3}
\end{figure*}


\begin{figure*}[h]
    \centering
    \includegraphics[width=0.75\linewidth]{Chameleon_cm.pdf}
    \includegraphics[width=0.75\linewidth]{Chameleon_hersch_col.pdf}
    \caption{The same as Figure~\ref{fig:afgl490}, but now for the Chamaeleon region, which is part of the test set. 
    }
    \label{fig:chamaeleon}
    
\end{figure*}


\begin{figure*}[h]
    \centering
    \includegraphics[width=0.75\linewidth]{CrA_cm.pdf}
    \includegraphics[width=0.75\linewidth]{CrA_hersch_col.pdf}
    \caption{The same as Figure~\ref{fig:afgl490}, but now for the Corona Australis region, which is part of set used to define training YSOs. 
    }
    \label{fig:cra}
\end{figure*}


\begin{figure*}[h]
    \centering
    \includegraphics[width=0.75\linewidth]{Cygnus_X_cm.pdf}
    \includegraphics[width=0.75\linewidth]{Cygnus_X_hersch_col.pdf}
    \caption{The same as Figure~\ref{fig:afgl490}, but now for the Cygnus X region, which is excluded from both test and training sets. 
    }
    \label{fig:cygnusx}
\end{figure*}


\begin{figure*}[h]
    \centering
    \includegraphics[width=0.75\linewidth]{GGD4_CB34_cm.pdf}
    \includegraphics[width=0.75\linewidth]{GGD4_CB34_hersch_col.pdf}
    \caption{The same as Figure~\ref{fig:afgl490}, but now for the GGD4 CB34 region, which is part of the test set. The Spitzer observations are at wide enough separation to require separating the fields into two subplots for better visualization.    }
    \label{fig:ggd4_cb34}
\end{figure*}


\begin{figure*}[h]
    \centering
    \includegraphics[width=0.75\linewidth]{IC_5146_cm.pdf}
    \includegraphics[width=0.75\linewidth]{IC_5146_hersch_col.pdf}
    \caption{The same as Figure~\ref{fig:afgl490}, but now for the IC 5146 region, which is part of the test set. 
    }
    \label{fig:ic5146}
\end{figure*}


\begin{figure*}[h]
    \centering
    \includegraphics[width=0.75\linewidth]{IRAS_20050+2720_cm.pdf}
    \includegraphics[width=0.75\linewidth]{IRAS_20050+2720_hersch_col.pdf}
    \caption{The same as Figure~\ref{fig:afgl490}, but now for the IRAS 20050+2720 region, which is part of the test set.}
    \label{fig:iras20050}
\end{figure*}


\begin{figure*}[h]
    \centering
    \includegraphics[width=0.75\linewidth]{L988_cm.pdf}
    \includegraphics[width=0.75\linewidth]{L988_hersch_col.pdf}
    \caption{The same as Figure~\ref{fig:afgl490}, but now for the L 988 region, which is part of the test set. 
   }
    \label{fig:l988}
\end{figure*}


\begin{figure*}[h]
    \centering
    \includegraphics[width=0.75\linewidth]{Lupus_cm.pdf}
    \includegraphics[width=0.9\linewidth]{Lupus_hersch_col.pdf}
    \caption{The same as Figure~\ref{fig:afgl490}, but now for the Lupus region, which is part of the test set. The Spitzer observations are at wide enough separation to require separating the fields into two subplots for better visualization.
    }
    \label{fig:lupus}
\end{figure*}


\begin{figure*}[h]
    \centering
    \includegraphics[width=0.75\linewidth]{Mon_OB1_cm.pdf}
    \includegraphics[width=0.75\linewidth]{Mon_OB1_hersch_col.pdf}
    \caption{The same as Figure~\ref{fig:afgl490}, but now for the Mon OB1 region, which is part of the test set. 
    }
    \label{fig:monob1}
\end{figure*}


\begin{figure*}[h]
    \centering
    \includegraphics[width=0.75\linewidth]{Mon_R2_cm.pdf}
    \includegraphics[width=0.75\linewidth]{Mon_R2_hersch_col.pdf}
    \caption{The same as Figure~\ref{fig:afgl490}, but now for the Mon R2 region, which is part of the test set. }
    \label{fig:monr2}
\end{figure*}


\begin{figure*}[h]
    \centering
    \includegraphics[width=0.75\linewidth]{Musca_cm.pdf}
    \includegraphics[width=0.75\linewidth]{Musca_hersch_col.pdf}
    \caption{The same as Figure~\ref{fig:afgl490}, but now for the Musca region, which is part of the test set. 
    }
    \label{fig:musca}
\end{figure*}


\begin{figure*}[h]
    \centering
    \includegraphics[width=0.75\linewidth]{NGC_7129_cm.pdf}
    \includegraphics[width=0.75\linewidth]{NGC_7129_hersch_col.pdf}
    \caption{The same as Figure~\ref{fig:afgl490}, but now for the NGC 7129 region, which is part of the test set. 
    }
    \label{fig:ngc7129}
\end{figure*}


\begin{figure*}[h]
    \centering
    \includegraphics[width=0.75\linewidth]{North_America_Nebula_cm.pdf}
    \includegraphics[width=0.75\linewidth]{North_America_Nebula_hersch_col.pdf}
    \caption{The same as Figure~\ref{fig:afgl490}, but now for the North America Nebula, which is part of the test set. }
    \label{fig:northamerica}
\end{figure*}


\begin{figure*}[h]
    \centering
    \includegraphics[width=0.75\linewidth]{Ophiuchus_cm.pdf}
    \includegraphics[width=0.75\linewidth]{Ophiuchus_hersch_col.pdf}
    \caption{The same as Figure~\ref{fig:afgl490}, but now for Ophiuchus, which is part of set used to define training YSOs. }
    \label{fig:ophiuchus}
\end{figure*}


\begin{figure*}[h]
    \centering
    \includegraphics[width=0.75\linewidth]{Orion_A_cm.pdf}
    \includegraphics[width=0.75\linewidth]{Orion_A_hersch_col.pdf}
    \caption{The same as Figure~\ref{fig:afgl490}, but now for Orion A, which is part of set used to define training YSOs. }
    \label{fig:oriona}
\end{figure*}


\begin{figure*}[h]
    \centering
    \includegraphics[width=0.75\linewidth]{Orion_B_cm.pdf}
    \includegraphics[width=0.75\linewidth]{Orion_B_hersch_col.pdf}
        \caption{The same as Figure~\ref{fig:afgl490}, but now for Orion B, which is part of set used to define training YSOs. }
    \label{fig:orionb}
\end{figure*}


\begin{figure*}[h]
    \centering
    \includegraphics[width=0.75\linewidth]{Perseus_cm.pdf}
    \includegraphics[width=0.75\linewidth]{Perseus_hersch_col.pdf}
    \caption{The same as Figure~\ref{fig:afgl490}, but now for the Perseus region, which is part of the test set. 
    }
    \label{fig:perseus}
\end{figure*}


\begin{figure*}[h]
    \centering
    \includegraphics[width=0.75\linewidth]{Pipe_cm.pdf}
    \includegraphics[width=0.75\linewidth]{Pipe_hersch_col.pdf}
    \caption{The same as Figure~\ref{fig:afgl490}, but now for the Pipe region, which is excluded from both test and training sets. NOTE: there is no estimate for the contamination rate by field stars, which, though generally easy to distinguish from YSOs, becomes significant when looking directly into the Galactic plane, as is done here.}
    % \caption{Confusion matrix for Pipe (excluded from test and training).
    % \bc{Contours are for 2,5,10,25}. NOTE: there is no estimate for the contamination rate by field stars, which, though generally easy to distinguish from YSOs, becomes significant when looking directly into the Galactic plane, as is done here.}
    \label{fig:pipe}
\end{figure*}


\begin{figure*}[h]
    \centering
    \includegraphics[width=0.75\linewidth]{S131_cm.pdf}
    \includegraphics[width=0.75\linewidth]{S131_hersch_col.pdf}
    \caption{The same as Figure~\ref{fig:afgl490}, but now for the S 131 region, which is part of the test set. 
    }
    \label{fig:s131}
\end{figure*}


\begin{figure*}[h]
    \centering
    \includegraphics[width=0.75\linewidth]{S140_cm.pdf}
    \includegraphics[width=0.75\linewidth]{S140_hersch_col.pdf}
    \caption{The same as Figure~\ref{fig:afgl490}, but now for the S 140 region, which is part of the test set. 
    }
    \label{fig:s140}
\end{figure*}


\begin{figure*}[h]
    \centering
    \includegraphics[width=0.75\linewidth]{S171_cm.pdf}
    \includegraphics[width=0.75\linewidth]{S171_hersch_col.pdf}
    \caption{The same as Figure~\ref{fig:afgl490}, but now for the S 171 region, which is part of the test set. 
    }
    \label{fig:s171}
\end{figure*}


\begin{figure*}[h]
    \centering
    \includegraphics[width=0.75\linewidth]{Scorpius_cm.pdf}
    \includegraphics[width=0.75\linewidth]{Scorpius_hersch_col.pdf}
    \caption{The same as Figure~\ref{fig:afgl490}, but now for the Scorpius region, which is part of the test set. The Spitzer observations are at wide enough separation to require separating the fields into two subplots for better visualization.}
    \label{fig:scorpius}
\end{figure*}


\begin{figure*}[h]
    \centering
    \includegraphics[width=0.75\linewidth]{Taurus_cm.pdf}
    \includegraphics[width=0.75\linewidth]{Taurus_hersch_col.pdf}
    \caption{The same as Figure~\ref{fig:afgl490}, but now for Taurus, which is part of the set used to define training YSOs. The Spitzer observations are at wide enough separation to require separating the fields into multiple subplots for better visualization.}
    \label{fig:taurus}
\end{figure*}


\begin{figure*}[h]
    \centering
    \includegraphics[width=0.75\linewidth]{Vela_D_cm.pdf}
    \includegraphics[width=0.75\linewidth]{Vela_D_hersch_col.pdf}
    \caption{The same as Figure~\ref{fig:afgl490}, but now for the Vela D region, which is part of the test set. 
    }
    \label{fig:velad}
\end{figure*}
